The Maass Space for Paramodular Groups

In this paper we describe a characterization for the Maass space associated with the paramodular group of degree $2$ and squarefree level $N$. As an application we show that the Maass space is invariant under all Hecke operators. As a consequence we conclude that the associated Siegel-Eisenstein series belongs to the Maass space.

==> bibliography_krieg <==
%bibliography.bib

%%%%%  von Herrn Krieg
@book{A,
	author = {{Andrianov, A.N.}},
	year	= {1987},
	title	= {{Quadratic Forms and Hecke Operators}},
	publisher = {{Springer-Verlag, Berlin}},
	series = {{Grundl. Math. Wiss.}},	
	volume = {286},
}
@article{BBK,
	author	= {{B\"ocherer, S., J.H. Bruinier} and W. Kohnen},
	year	= {1999},
	journal = {Math. Ann.},
	volume	= {313},
	title	= {{Non-vanishing of scalar products of Fourier-Jacobi coefficients of Siegel cusp forms}},
	pages	= {1--13},
}
@article{Bo,
	author	= {{Borcherds, R.}},
	journal = {Invent. Math.},
	volume    = {132},
        year  =  {1998},
	title	= {{Automorphic forms with singularities on Grassmannians.}},
	pages ={491--562},
} 
@article{BK,
	author	= {{Brumer, A. and K. Kramer}},
	journal = {Trans. Am. Math. Soc.},
	volume    = {366},
        year  =  {2014},
	title	= {{Paramodular abelian varieties of odd conductor.}},
	pages ={2463--2516},
} 
@book{EZ,
	author	= {{Eichler, M. and D. Zagier}},
	year	= {1985},
	title	= {{The Theory of Jacobi Forms}},
	publisher = {Birkhäuser, Boston, Basel, Stuttgart},
}
@article{E,
	author	= {{Elstrodt, J.}},
	journal = {Math. Ann.},
	volume    = {268},
        year  =  {1984},
	title	= {{Eine Charakterisierung der Eisenstein-Reihe zur Siegelschen Modulgruppe}},
	pages ={473--474},
} 
@book{F,
	author = {{Freitag, E.}},
	year	= {1983},
	title	= {{Siegelsche Modulfunktionen}},
	series	= {{Grundl. Math. Wiss.}},
	publisher = {Springer-Verlag, Berlin},
	volume = {254},
}
@article{GK,
	author	= {{Gallenkämper, J.} and A. Krieg},
	journal = {},
	title	= {{The Hecke algebras for the orthogonal group $SO(2,3)$ and the paramodular group of degree $2$}},
	note	= {ArXiv:1710.09156},
}
@article{GHK,
	author	= {{Gallenkämper, J., B. Heim} and A. Krieg},
	year	= {2016},
	journal = {Int. J. Math.},
	volume	= {27},
	title	= {{The Maaß space and Hecke operators}},
	pages	= {1--8},
	note	= {ID 1650039},
}
@incollection{G1,
	author	= {{Gritsenko, V.A.}},
	year	= {1995},
	booktitle	= {Number theory},
	editor	= {S. David and others},
	edition = {{Cambridge Univ. Press}},
	location = {Cambridge},
	volume	= {},
	title	= {{Arithmetical lifting and its applications.}},
	pages	= {103--126},
}
@article{G2,
	author	= {{Gritsenko, V.A.}},
	year	= {1995},
	journal = {Math. Gottingensis},
	volume	= {12},
	title	= {{Modulformen zur Paramodulgruppe und Modulr{\"a}ume der abelschen Variet{\"a}ten}},
	pages	= {1--89},
}
@incollection{G3,
	author	= {{Gritsenko, V.A.}},
	year	= {1995},
	booktitle	= {Abelian varieties },
	editor	= {W. Barth and others},
	edition = {{Walter de Gruyter}},
	location = {Cambridge},
	volume	= {},
	title	= {{Irrationality of the moduli spaces of polarized abelian surfaces.}},
	pages	= {63--81},
}
@article{H,
	author	= {{Heim, B.}},
	year	= {2010},
	journal = {Int. J. Math. Math. Sci.},
	volume	= {23},
	title	= {{On the Spezialschar of Maass}},
	pages	= {1--13},
}
@article{HM1,
	author	= {{Heim, B. and S. Murase}},
	year	= {2012},
	journal = {Int. J. Math.},
	volume	= {23},
	title	= {{A characterization of the Maass space on $O(2,m+2)$ by symmetries}},
	pages	= {1--13},
	note	= {ID 125006},
}
@article{K2,
	author	= {{Krieg, A.}},
	year	= {1990},
	journal = {Mem. Am. Math. Soc.},
	volume	= {435},
	title	= {{Hecke algebras}},
	pages	= {},
}
@incollection{K1,
	author	= {{Krieg, A.}},
	year	= {2016},
	booktitle	= {Dynamical systems, number theory and applications},
	editor	= {T. Hagen and others},
	edition = {{World Scientific}},
	location = {},
	volume	= {},
	title	= {{Integral orthogonal groups}},
	pages	= {177--195},
}
@article{O,
	author	= {{Oda, T.}},
	journal = {Math. Ann.},
	year    = {1977},
	volume  = {231},
	title	= {{On modular forms associated with indefinite quadratic forms of signature $(2,n-2)$}},
	pages = {97--144},
}
@article{PY,
	author	= {{Poor, C. and D. Yuen}},
	journal = {J. Korean Math. Soc.},
	year    = {2013},
	volume  = {50},
	title	= {{The cusp structure of the paramodular groups of degree two.}},
	pages = {445--464},
}
@inproceedings{RS1,                              
	author	= {{Roberts, B. and R. Schmidt}},
	year	= {2006},
	booktitle	= {Automorphic forms and zeta functions},
	editor	= {Proc. Conf. Mem. Tsuneo Arakawa},
	edition = {World Scientific},
	volume	= { },
	title	= {{On modular forms for the paramodular group.}},
	pages	= {},
}
@book{RS2,
	author = {{Roberts, B. and R. Schmidt}},
	year	= {2007},
	title	= {{Local newforms for $GSp(4)$}},
	series	= {{Lect. Notes Math.}},
	publisher = {Springer-Verlag, Berlin},
	volume = {1918},
}
@article{RT,
	author	= {{Ryan, N.C. and G. Tornaria}},
	journal = {Int. J. Number Theory},
	volume    = {7},
        year  =  {2011},
	title	= {{A Böcherer-type conjecture for paramodular forms.}},
	pages ={1395--1411},
}
@article{Si,
	author	= {{Siegel, C.L.}},
	journal = {Nachr. Akad. Wiss. Göttingen, Math.-phys. Kl.},
	volume    = {25},
        year  =  {1964},
	title	= {{Moduln Abelscher Funktionen.}},
	pages ={365--427},
} 
@article{Su,
	author	= {{Sugano, T.}},
	journal = {Comm. Math. Univ. St. Pauli},
	volume    = {44},
        year  =  {1994},
	title	= {{Jacobi Forms and the Theta Lifting.}},
	pages ={1--57},
} 

